3-Lead to 12-Lead ECG Reconstruction: A Novel AI-based Spatio-Temporal Method

Diagnosis of cardiovascular diseases usually relies on the widely used standard 12-Lead (S12) ECG system. However, such a system could be bulky, too resource-intensive, and too specialized for personalized home-based monitoring. In contrast, clinicians are generally not trained on the alternative proposal, i.e., the reduced lead (RL) system. This necessitates mapping RL to S12. In this context, to improve upon traditional linear transformation (LT) techniques, artificial intelligence (AI) approaches like long short-term memory (LSTM) networks capturing non-linear temporal dependencies, have been suggested. However, LSTM does not adequately interpolate spatially (in 3D). To fill this gap, we propose a combined LSTM-UNet model that also handles spatial aspects of the problem, and demonstrate performance improvement. Evaluated on PhysioNet PTBDB database, our LSTM-UNet achieved a mean R^2 value of 94.37%, surpassing LSTM by 0.79% and LT by 2.73%. Similarly, for PhysioNet INCARTDB database, LSTM-UNet achieved a mean R^2 value of 93.91%, outperforming LSTM by 1.78% and LT by 12.17%.

==> 3D.tex <==


\begin{figure}
\includegraphics[width=0.5\columnwidth]{3D.eps}
\centering
\caption{Schematic presentation of the lead vectors of the Standard 12-lead ECG system}
\label{S12_R3L_3D}
\end{figure}

==> ptbdb_HC.tex <==




\begin{table}
\begin{center}
\begin{small}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{4pt}

\caption{Mean $R^2$, $r_x$ and $ndtw$ between the original and the reconstructed ECG signal obtained for HC patients in PTBDB}

\begin{tabular}{|c|ccc|ccc|cc|}
\hline
\cline{2-9}
& \multicolumn{3}{c|}{$R^2$}
& \multicolumn{3}{c|}{$r_x$} & \multicolumn{2}{c|}{$ndtw$} 
\\
\cline{2-9}
lead & a & b & c & a & b & c & b & c \\
\hline
III & - &0.976 & 95.27 & -  & 0.976& 0.936 & 95.27 & 0.976\\
avR & - & 0.936 & 95.27 & - & 86.38 & 0.936 & 95.27 & 0.976\\
avL & - & 0.936 & 95.27 & -& 86.38 & 0.936 & 95.27 & 0.976\\
avF & - & 0.936 & 95.27 & - & 86.38 & 0.936 & 95.27 & 0.976\\
V1 & 94.69 & 0.936 & 95.91 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V3 & 96.52 & 0.940 & 97.49 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V4 & 91.83 & 0.922 & 95.66 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V5 & 93.53 & 0.921 & 97.11 & 0.965 & 86.38 & 0.936 & 95.27 & 0.976\\
V6 & 94.69 & 0.893 &96.81 & 0.973 & 86.38 & 0.936 & 95.27 & 0.976\\
%\rule{0pt}{15pt}
\hline
Avg & 90.89 & 96.59 & 0.972 & 83.75 & 0.922 & 94.38 & 0.972 & 0.976\\


\hline
\end{tabular}
\label{final_results}
\end{small}


\end{center}
\end{table}

==> ptbdb_HY.tex <==




\begin{table}
\begin{center}
\begin{small}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{4pt}

\caption{Mean $R^2$, $r_x$ and $ndtw$ between the original and the reconstructed ECG signal obtained for HY patients in PTBDB}

\begin{tabular}{|c|ccc|ccc|cc|}
\hline
\cline{2-9}
& \multicolumn{3}{c|}{$R^2$}
& \multicolumn{3}{c|}{$r_x$} & \multicolumn{2}{c|}{$ndtw$} 
\\
\cline{2-9}
lead & a & b & c & a & b & c & b & c \\
\hline
III & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avR & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avL & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avF & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V1 & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V3 & 86.91 & 0.940 & 94.40 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V4 & 83.61 & 0.922 & 94.35 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V5 & 83.74 & 0.921 & 93.17 & 0.965 & 86.38 & 0.936 & 95.27 & 0.976\\
V6 & 78.11 & 0.893 & 94.71 & 0.973 & 86.38 & 0.936 & 95.27 & 0.976\\
%\rule{0pt}{15pt}
\hline
Avg & 83.75 & 0.922 & 94.38 & 0.972 & 83.75 & 0.922 & 94.38 & 0.972\\


\hline
\end{tabular}
\label{final_results}
\end{small}


\end{center}
\end{table}

==> ptbdb_MI.tex <==






\begin{table}
\begin{center}
\begin{small}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{4pt}

\caption{Mean $R^2$, $r_x$ and $ndtw$ between the original and the reconstructed ECG signal obtained for MI patients in PTBDB}

\begin{tabular}{|c|ccc|ccc|cc|}
\hline
\cline{2-9}
& \multicolumn{3}{c|}{$R^2$}
& \multicolumn{3}{c|}{$r_x$} & \multicolumn{2}{c|}{$ndtw$} 
\\
\cline{2-9}
lead & a & b & c & a & b & c & b & c \\
\hline
III & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avR & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avL & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avF & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V1 & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V3 & 86.91 & 0.940 & 94.40 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V4 & 83.61 & 0.922 & 94.35 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V5 & 83.74 & 0.921 & 93.17 & 0.965 & 86.38 & 0.936 & 95.27 & 0.976\\
V6 & 78.11 & 0.893 & 94.71 & 0.973 & 86.38 & 0.936 & 95.27 & 0.976\\
%\rule{0pt}{15pt}
\hline
Avg & 83.75 & 0.922 & 94.38 & 0.972 & 83.75 & 0.922 & 94.38 & 0.972\\


\hline
\end{tabular}
\label{final_results}
\end{small}


\end{center}
\end{table}

==> ptbdb_ND.tex <==



\begin{table}
\begin{center}
\begin{small}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{4pt}

\caption{Mean $R^2$, $r_x$ and $ndtw$ between the original and the reconstructed ECG signal obtained for ND patients in PTBDB}

\begin{tabular}{|c|ccc|ccc|cc|}
\hline
\cline{2-9}
& \multicolumn{3}{c|}{$R^2$}
& \multicolumn{3}{c|}{$r_x$} & \multicolumn{2}{c|}{$ndtw$} 
\\
\cline{2-9}
lead & a & b & c & a & b & c & b & c \\
\hline
III & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avR & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avL & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avF & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V1 & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V3 & 86.91 & 0.940 & 94.40 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V4 & 83.61 & 0.922 & 94.35 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V5 & 83.74 & 0.921 & 93.17 & 0.965 & 86.38 & 0.936 & 95.27 & 0.976\\
V6 & 78.11 & 0.893 & 94.71 & 0.973 & 86.38 & 0.936 & 95.27 & 0.976\\
%\rule{0pt}{15pt}
\hline
Avg & 83.75 & 0.922 & 94.38 & 0.972 & 83.75 & 0.922 & 94.38 & 0.972\\


\hline
\end{tabular}
\label{final_results}
\end{small}


\end{center}
\end{table}

==> ptbdb_VA.tex <==



\begin{table}
\begin{center}
\begin{small}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{4pt}

\caption{Mean $R^2$, $r_x$ and $ndtw$ between the original and the reconstructed ECG signal obtained for VA patients in PTBDB}

\begin{tabular}{|c|ccc|ccc|cc|}
\hline
\cline{2-9}
& \multicolumn{3}{c|}{$R^2$}
& \multicolumn{3}{c|}{$r_x$} & \multicolumn{2}{c|}{$ndtw$} 
\\
\cline{2-9}
lead & a & b & c & a & b & c & b & c \\
\hline
III & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avR & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avL & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
avF & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V1 & 86.38 & 0.936 & 95.27 & 0.976 & 86.38 & 0.936 & 95.27 & 0.976\\
V3 & 86.91 & 0.940 & 94.40 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V4 & 83.61 & 0.922 & 94.35 & 0.972 & 86.38 & 0.936 & 95.27 & 0.976\\
V5 & 83.74 & 0.921 & 93.17 & 0.965 & 86.38 & 0.936 & 95.27 & 0.976\\
V6 & 78.11 & 0.893 & 94.71 & 0.973 & 86.38 & 0.936 & 95.27 & 0.976\\
%\rule{0pt}{15pt}
\hline
Avg & 83.75 & 0.922 & 94.38 & 0.972 & 83.75 & 0.922 & 94.38 & 0.972\\


\hline
\end{tabular}
\label{final_results}
\end{small}


\end{center}
\end{table}
